Probabilistic DAG Search

Exciting contemporary machine learning problems have recently been phrased in the classic formalism of tree search -- most famously, the game of Go. Interestingly, the state-space underlying these sequential decision-making problems often posses a more general latent structure than can be captured by a tree. In this work, we develop a probabilistic framework to exploit a search space's latent structure and thereby share information across the search tree. The method is based on a combination of approximate inference in jointly Gaussian models for the explored part of the problem, and an abstraction for the unexplored part that imposes a reduction of complexity ad hoc. We empirically find our algorithm to compare favorably to existing non-probabilistic alternatives in Tic-Tac-Toe and a feature selection application.

==> figures/selected_pixels/labeled_pixels.tex <==
% This file was created by tikzplotlib v0.9.4.
\begin{tikzpicture}

\begin{groupplot}[group style={group size=3 by 3}]
\nextgroupplot[
height=4.5cm,
minor xtick={},
minor ytick={},
tick pos=both,
width=4.5cm,
xmin=-0.5, xmax=27.5,
xtick=\empty,
y dir=reverse,
ymin=-0.5, ymax=27.5,
ytick=\empty
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=27.5, ymin=27.5, ymax=-0.5] {./figures/selected_pixels/labeled_pixels_zero.png};
\node[anchor=west] (source) at (axis cs:16,7);
\node (destination) at (axis cs:16,10){};
\draw[->](source)--(destination);
\draw (axis cs:16,7) node[
  scale=1,
  anchor=base west,
  text=yellow,%green,%!50.1960784313725!black,
  rotate=0.0
]{0};
\draw (axis cs:9,10) node[
  scale=1,
  anchor=base west,
  text=green!50.1960784313725!black,
  rotate=0.0
]{1};
\draw (axis cs:19,11) node[
  scale=1,
  anchor=base west,
  text=green!50.1960784313725!black,
  rotate=0.0
]{2};
\draw (axis cs:9,14) node[
  scale=1,
  anchor=base west,
  text=green!50.1960784313725!black,
  rotate=0.0
]{3};
\draw (axis cs:13,14) node[
  scale=1,
  anchor=base west,
  text=green!50.1960784313725!black,
  rotate=0.0
]{4};
\draw (axis cs:11,17) node[
  scale=1,
  anchor=base west,
  text=green!50.1960784313725!black,
  rotate=0.0
]{5};
\draw (axis cs:8,20) node[
  scale=1,
  anchor=base west,
  text=green!50.1960784313725!black,
  rotate=0.0
]{6};
\draw (axis cs:11,20) node[
  scale=1,
  anchor=base west,
  text=green!50.1960784313725!black,
  rotate=0.0
]{7};
\draw (axis cs:9,22) node[
  scale=1,
  anchor=base west,
  text=green!50.1960784313725!black,
  rotate=0.0
]{8};
\draw (axis cs:15,22) node[
  scale=1,
  anchor=base west,
  text=green!50.1960784313725!black,
  rotate=0.0
]{9};
\end{groupplot}

\end{tikzpicture}

